EDUCE: Explaining model Decisions through Unsupervised Concepts Extraction

Providing explanations along with predictions is crucial in some text processing tasks. Therefore, we propose a new self-interpretable model that performs output prediction and simultaneously provides an explanation in terms of the presence of particular concepts in the input. To do so, our model's prediction relies solely on a low-dimensional binary representation of the input, where each feature denotes the presence or absence of concepts. The presence of a concept is decided from an excerpt i.e. a small sequence of consecutive words in the text. Relevant concepts for the prediction task at hand are automatically defined by our model, avoiding the need for concept-level annotations. To ease interpretability, we enforce that for each concept, the corresponding excerpts share similar semantics and are differentiable from each others. We experimentally demonstrate the relevance of our approach on text classification and multi-sentiment analysis tasks.

==> architectures.tex <==
\section{Architectures}
\label{sec:archi}
Our model can be instantiated with multiple neural network architectures depending on the nature of the task to solve. Since we are facing sequences of vectors (i.e 2D tensors) for text data, and 3D tensors for images, we rely on a generic architecture based on convolutions. We describe below the architecture and the inference process in the case of text data, but the extension to 3D tensors for image data is straightforward.

Every word in the input is represented as an pre-trained word embedding vector, therefore the input is a 2D tensor of dimensions number of words $\times$ embedding size. Let us consider an input text $x$, and that each sub-part $s$ of $x$ is a combination of 2 consecutive words. First, we build the probability distribution for each concept, over all sub-parts, that is $p(s_c|x,c)$. To do so, we feed $x$ to a linear layer of dimension $d \times C$ where $d$ is the size of a sub-part of $x$. In our example, this corresponds to twice the word embedding size, as each sub-part is composed of 2 consecutive words.

The linear layer returns a score over all subparts, for each concept independently, giving a 2D tensor denoted $M_S$ in Figure \ref{fig:archiex} of dimensions $C \times |S_x|$ where $|S_x|$ is the number of sub-parts in $x$ and $C$ the number of concepts. It is followed by a softmax non-linearity over the possible sub-parts, for each concept (that is, for each row of the tensor ): this gives $p(s_c|x,c)$. For each concept, that is, we sample a sub-part $s_c \sim p(s_c|x,c)$. Note that a sub-part can belong to multiple concept or be overlapping.

As a second step, we process independently each one of the unique selected sub-parts for every concept, $s_c$, to obtain a score corresponding to the presence / absence of that concept, that is $p(h|s_c,c)$. Specifically, we take the dot product of a weight vector $w_c \in \mathbb{R}^d$ per concept with the selected sub-part, followed by a sigmoid activation function, as follows:
\begin{equation}
p(h|s_c,c) = \text{sigmoid}(\sum_{d=1}^{D} w_{c,d} s_{c,d})
\end{equation}


==> experiments.tex <==
\subsection{Text classification experiments}
\label{sec:expe}

\textbf{Experimental setting} For our experiment on text data we use the DBpedia ontology classification dataset and the AGNews topic classification dataset both created by \citep{Zhang:LeCun:2015}. The DBpedia ontology classification dataset was constructed by picking $14$ non-overlapping categories from DBpedia 2014 \citep{Lehmann:etal:2014}. We subsample $56,000$ examples of the train dataset for training, and $56,000$ for validation. For testing, we subsample $7,000$ of the $70,000$ examples in the test dataset (using stratified sampling). The AGNews topic classification dataset was constructed from the AG dataset by choosing 4 largest categories. We divide the training set into two sets: $84,000$ training samples and $24,000$ validation samples. We test on the full test dataset composed of $7,600$ samples. In both datasets the title of the abstract or article is available but we do not use it. We use pre-trained word vectors trained on Common Crawl \citep{Grave:etal:2018}, and keep them fixed. Code for pre-processing of the datasets will be released along the code for our model. We consider patterns $s$ as all sets composed of $3$ consecutive words\footnote{In our early experiments we considered flexible number of words in the patterns but performance were poorer, we consider this as direction for future research.}. Therefore, sampling a pattern is equivalent to the sampling of its start word resulting in an efficient sampling model.  The ``Classic" model is a Bidirectional LSTM while our model is based on convolutional layers. We monitor final prediction accuracy on the validation set and report results on the test set. For each set of hyperparameters, we run $5$ different random seeds. We explore three different number of concepts: $C=5$, $C=10$ and $C=20$, and we evidently consider each value of $C$ separately as $C$ directly affects the concept classifier's base performance. Details on the range of hyperparameters explored, the training procedure and size of the architecture is in  supplementary material Section \ref{sec:expesupp}.


==> learning.tex <==
\section{Learning Algorithm}

\paragraph{Gradient w.r.t. $\theta$} The gradient of our objective function for a single input $x$, w.r.t. the final classifier parameters writes as:
\begin{flalign}
\nabla_{\theta}\mathcal{L}(x) &= \nabla_{\theta}\mathcal{L}^{classif}(x) = \nabla_{\theta}\mathbb{E}_{\substack{s_c(x) \sim \gamma_c(s|x) \forall c \\ h_c(x) \sim \alpha_c(s_c(x)) \forall c }} [ \Delta ( f(h(x)),y)] \nonumber \\
&= \mathbb{E}_{\substack{s_c(x) \sim \gamma_c(s|x) \forall c \\ h_c(x) \sim \alpha_c(s_c(x)) \forall c }} [ \nabla_{\theta}\Delta ( f(h(x)),y)]
\end{flalign}

\paragraph{Gradient w.r.t. $\theta_c$} The gradient of our objective function for a single input $x$, w.r.t. the concepts classifier parameters writes as:
\begin{flalign}
\nabla_{\theta_c}\mathcal{L}(x) &= \lambda_c \nabla_{\theta_c} \mathcal{L}^{concept}(x) = \lambda_c \nabla_{\theta_c} \frac{1}{C} \sum\limits_{c} \mathbb{E}_{\substack{s_c(x) \sim \gamma_c(s|x)\\ h_c \sim \alpha_c(s_c(x))}}[h_c(x)\Delta'(g(s_c(x)),c)]\nonumber \\
&=\lambda_c \frac{1}{C} \sum\limits_{c} \mathbb{E}_{\substack{s_c(x) \sim \gamma_c(s|x)\\ h_c \sim \alpha_c(s_c(x))}}[h_c(x)\nabla_{\theta_c} \Delta'(g(s_c(x)),c)]
\end{flalign}

\paragraph{Gradient w.r.t. $\theta_h$}


\begin{flalign}
&\nabla_{\theta_h}\mathbb{E}_{x} [\mathcal{L}^{classif}(\alpha,\gamma,f,x,y) + \lambda_c \mathcal{L}^{concept}(\delta,x)]\nonumber \\
&=\nabla_{\theta_h}\mathbb{E}_{\substack{s_c(x) \sim \gamma_c(s|x) \forall c \\ h_c(x) \sim \alpha_c(s_c(x)) \forall c }} [ \Delta ( f(h(x)),y)+ \lambda_c \frac{1}{C} \sum\limits_{c} h_c(x)\Delta'(g(s_c(x)),c)]\nonumber \\
&\mathrel{\widehat{=}}\mathbb{E}_{\substack{s_c(x) \sim \gamma_c(s|x) \forall c \\ h_c(x) \sim \alpha_c(s_c(x)) \forall c }} [  \Big(\Delta ( f(h(x)),y)+ \lambda_c \frac{1}{C} \sum\limits_{c} h_c(x)\Delta'(g(s_c(x)),c)\Big)\nabla_{\theta_h}\log p_{\theta_h} (h(x))]
\end{flalign}
% and the overall gradient w.r.t. $\theta_h$ writes as:
% \begin{flalign}
% \nabla_{\theta_h} \mathcal{L}(x)&=\mathbb{E}_{e(x)}[\mathbb{E}_{h(x)}[\Delta(\langle \theta ; h(x) \rangle; y)\nabla_{\theta_h}  \log p_{\theta_h} (h(x))]] \nonumber \\
% &\quad+ \frac{\lambda_c}{H}\sum\limits_{i=1}^H \nabla_{\theta_h} \hat{h}_i(x) \mathbb{E}_{e_i(x)}[\Delta'(\langle \theta_c ; e_i(x) \rangle,i)]
% \end{flalign}
% The concept extractor is defined as follows. First, a recurrent architecture parses the text input and embeds it into a hidden representation. Then, probabilities for the start and stop words of the patch are computed from the hidden representations. The patches are computed as the mean of extracted words vectors.
\paragraph{Gradient w.r.t. $\theta_s$}
In our experiment on text data, concept instances $s_c(x)$ correspond to part of sequences. For each patch $s_c(x)$, the start and stop words of the instance are discrete random variables, which we denote jointly as $w_c(x)$. The parameters $\theta_s$ refer collectively to both the differentiable (embedding of the text input by the recurrent architecture) and non-differentiable (sampling of the start and stop words) operations. Again, we employ the REINFORCE algorithm.

\begin{flalign}
&\nabla_{\theta_s}\mathbb{E}_{x} [\mathcal{L}^{classif}(\alpha,\gamma,f,x,y) + \lambda_c \mathcal{L}^{concept}(\delta,x)]\nonumber \\
&=\nabla_{\theta_s}\mathbb{E}_{\substack{s_c(x) \sim \gamma_c(s|x) \forall c \\ h_c(x) \sim \alpha_c(s_c(x)) \forall c }} [ \Delta ( f(h(x)),y)+ \lambda_c \frac{1}{C} \sum\limits_{c} h_c(x)\Delta'(g(s_c(x)),c)]\nonumber \\
&\mathrel{\widehat{=}}\mathbb{E}_{\substack{s_c(x) \sim \gamma_c(s|x) \forall c \\ h_c(x) \sim \alpha_c(s_c(x)) \forall c }} [  \Big(\Delta ( f(h(x)),y)+ \lambda_c \frac{1}{C} \sum\limits_{c} h_c(x)\Delta'(g(s_c(x)),c)\Big)\nabla_{\theta_s}\log p_{\theta_s} (s_c(x))]
\end{flalign}
%
% \begin{flalign}
% \nabla_{\theta_s}\mathcal{L}^{classif}(x)\mathrel{\widehat{=}}\mathbb{E}_{e(x)}[\mathbb{E}_{h(x)}[\Delta(\langle \theta ; h(x) \rangle; y) (\nabla_{\theta_e} \log p_{\theta_h} (h(x)) + \nabla_{\theta_e}\log p_{\theta_e} (w(x))]]
% \end{flalign}
% \begin{flalign}
% \nabla_{\theta_e}\mathcal{L}^{concept}(x)=\frac{\lambda_c}{H}\sum\limits_{i=1}^H \nabla_{\theta_e} \hat{h}_i(x) \mathbb{E}_{e_i(x)} [\Delta'(\langle \theta_c ; e_i(x) \rangle; i)] +  \hat{h}_i(x) \nabla_{\theta_e} \mathbb{E}_{e_i(x)} [\Delta'(\langle \theta_c ; e_i(x) \rangle; i)]
% \end{flalign}
% where
% \begin{flalign}
% \nabla_{\theta_e} \mathbb{E}_{e_i(x)} [\Delta'(\langle \theta_c ; e_i(x) \rangle; i)]&\widehat{=}\hat{h}_i(x) \mathbb{E}_{e_i(x)} [\nabla_{\theta_e}\Delta'(\langle \theta_c ; e_i(x) \rangle; i)]\nonumber \\
% &\quad+\mathbb{E}_{e_i(x)} [\Delta'(\langle \theta_c ; e_i(x) \rangle; i) \nabla_{\theta_e} \log p_{\theta_e}(w_i(x))]
% \end{flalign}
%
% The overall gradient w.r.t $\theta_e$ writes as:
% \begin{flalign}
% \nabla_{\theta_e} \mathcal{L}(x) &=\mathbb{E}_{e(x)}[\mathbb{E}_{h(x)}[\Delta(\langle \theta ; h(x) \rangle; y) (\nabla_{\theta_e} \log p_{\theta_h} (h(x)) + \nabla_{\theta_e}\log p_{\theta_e} (e(x)))]] \nonumber \\
% &\quad+\frac{\lambda_c}{H}\sum\limits_{i=1}^H \nabla_{\theta_e} \hat{h}_i(x) \mathbb{E}_{e_i(x)} [\Delta'(\langle \theta_c ; e_i(x) \rangle; i)]\nonumber \\
% &\quad+\frac{\lambda_c}{H}\sum\limits_{i=1}^H\hat{h}_i(x)\mathbb{E}_{e_i(x)} [\nabla_{\theta_e}\Delta'(\langle \theta_c ; e_i(x) \rangle; i)]\nonumber \\
% &\quad+\frac{\lambda_c}{H}\sum\limits_{i=1}^H\hat{h}_i(x)\mathbb{E}_{e_i(x)} [\Delta'(\langle \theta_c ; e_i(x) \rangle; i) \nabla_{\theta_e} \log p_{\theta_e}(e_i(x))]
% \end{flalign}
% In our experiment on image data, patch extraction is a fully differentiable process, therefore the gradient is simply:
% \begin{flalign}
% \nabla_{\theta_e} \mathcal{L}(x) &=\mathbb{E}_{e(x)}[\mathbb{E}_{h(x)}[\Delta(\langle \theta ; h(x) \rangle; y) (\nabla_{\theta_e} \log p_{\theta_h} (h(x))] \nonumber \\
% &\quad+\frac{\lambda_c}{H}\sum\limits_{i=1}^H \nabla_{\theta_e} \hat{h}_i(x) \mathbb{E}_{e_i(x)} [\Delta'(\langle \theta_c ; e_i(x) \rangle; i)]\nonumber \\
% &\quad+\frac{\lambda_c}{H}\sum\limits_{i=1}^H\hat{h}_i(x)\mathbb{E}_{e_i(x)} [\nabla_{\theta_e}\Delta'(\langle \theta_c ; e_i(x) \rangle; i)]\nonumber \\
% \end{flalign}
\paragraph{Todo}
In that case, one has to use a bias reduction term resulting in the following gradient update rule:\todo{mention baseline in footnote}. \todo{Previously we mentioned two different solutions: We can also optimize our model using the straightthrough estimator proposed in \cite{XX}}. The two learning algorithms are tested in the experimental section. A complete implementation of the model is given at \url{http://XXXXXXXXXXXXX}.


==> resultext.tex <==
\section{Image classification experiments}
\label{sec:expe2}

Having assessed the relevance of our model on text data, we now turn to image data and explore if the EDUCE model is also able to extract meaningful concepts.

\textbf{Setting} We tackle image classification using MNIST \cite{Lecun:etal:98} to evaluate our approach, and results over the dataset are given in supplementary material. To further test the relevance of the patterns detected, we build a dataset where each image contains two randomly located of different labels. As we consider labels $0$ to $4$, there are 10 possible resulting categories that are the combination of the two digits label: $(0,1),(0,2),...,(3,4)$. We train  on $32,000$ generated images, and tested on $32,000$ different images. We achieve test final classification performance $96\%$ using $C=10$ concepts. Figure \ref{fig:m1} shows extracted patterns (not cherry picked) for the $10$ concepts, and the categories associated with the appearance of this concept. As in our experiments with text data, we can explain the model behavior: the model learns to extract single digits as patterns for different concepts, that are then combined to predict the final category.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.9\linewidth]{emnistc5.pdf}
\end{center}
\caption{Samples of patterns extracted for each concept. Under each concept, we show the categories associated with this concept}
\label{fig:m1}
\end{figure}

We also conduct experiments on a dataset composed of $224\times224$ RGB images split in $3$ categories: dogs, cats and birds\footnote{We construct this dataset by combining random images from the Caltech Bird 200-2011 dataset \citep{WahCUB_200_2011} with images of the cats-and-dogs Kaggle dataset \citep{KaggleDogVCat}} in equal proportion. We train on $3,000$ images and test on $3,000$ images. We build our model on top of a pretrained VGG-11 model \cite{Simonyan14c}. Figure 2 shows extracted patterns and associated categories. Final classification performance is $91.6\%$ with $10$ concepts. In Figure \ref{fig:m2} we plot extracted patterns for the $10$ concepts and report in Figure \ref{fig:m3} the weights of the final classifier. From these two figures, we can interpret the model's behavior: concept 8 and concept 9 show what differentiate a \emph{dog} from a \emph{cat} or a \emph{bird}, and support the classifier's prediction of the dog category. Figure \ref{fig:m4} shows the extracted patterns on random images. We can see that our model focuses on relevant parts of the images, similar to attention models.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.9\linewidth]{ebirdsp.pdf}
\end{center}
\caption{Samples of patterns extracted for each concept in the birds-cats-dogs dataset.}
\label{fig:m2}
\end{figure}

\begin{figure}[h!]
\begin{subfigure}[b]{0.45\textwidth}
        \centering \includegraphics[width=\textwidth]{ebirdss.pdf}
    \caption{Final Classifier weights, each column is a concept (0 to 9, from left to right) each row a final category. The lighter, the higher the weight is. Concepts 6 and 7 are associated to category 'Bird', Concept 1 and 4 to 'Cat' and concepts 8 and 9 to 'Dog'. }
  \label{fig:m3}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.45\textwidth}
        \centering \includegraphics[width=\textwidth]{ebirdsi.pdf}
        \caption{Examples of classified images (column 2 and 4) and corresponding extracted patterns (column 1 and 3) for concept detected as present.}
          \label{fig:m4}
    \end{subfigure}
\end{figure}

